Resource Allocation for Multi-User Downlink MISO OFDMA-URLLC Systems

This paper considers the resource allocation algorithm design for downlink multiple-input single-output (MISO) orthogonal frequency division multiple access (OFDMA) ultra-reliable low latency communication (URLLC) systems. To meet the stringent delay requirements of URLLC, short packet transmission is adopted and taken into account for resource allocation algorithm design. The resource allocation is optimized for maximization of the weighted system sum throughput subject to quality-of-service (QoS) constraints regarding the URLLC users' number of transmitted bits, packet error probability, and delay. Despite the non-convexity of the resulting optimization problem, the optimal solution is found via monotonic optimization. The corresponding optimal resource allocation policy can serve as a performance upper bound for sub-optimal low-complexity solutions. We develop such a low-complexity resource allocation algorithm to strike a balance between performance and complexity. Our simulation results reveal the importance of using multiple antennas for reducing the latency and improving the reliability of URLLC systems. Moreover, the proposed sub-optimal algorithm is shown to closely approach the performance of the proposed optimal algorithm and outperforms two baseline schemes by a considerable margin, especially when the users have heterogeneous delay requirements. Finally, conventional resource allocation designs based on Shannon's capacity formula are shown to be not applicable in MISO OFDMA-URLLC systems as they may violate the users' delay constraints.

==> a2.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{016}[cl][cl]{\matlabtextA $S_{1},K=4$}%
\psfrag{017}[cl][cl]{\matlabtextA $S_{1}$, $K=6$}%
\psfrag{018}[cl][cl]{\matlabtextA $S_{0}$, $K=6$}%
\psfrag{019}[cl][cl]{\matlabtextA Baseline scheme 2}%
\psfrag{020}[cl][cl]{\matlabtextA Proposed subopt. scheme}%
\psfrag{021}[cl][cl]{\matlabtextA Upper bound}%
\psfrag{022}[bc][bc]{\matlabtextA Average system sum throughput [bits/s/Hz]}%
\psfrag{023}[tc][tc]{\matlabtextA Number of antennas at the BS}%
\psfrag{024}[tl][tl]{\matlabtextA \begin{tabular}{@{}l@{}}Performance\\gain\end{tabular}}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $6$}%
\psfrag{001}[ct][ct]{\matlabtextA $7$}%
\psfrag{002}[ct][ct]{\matlabtextA $8$}%
\psfrag{003}[ct][ct]{\matlabtextA $9$}%
\psfrag{004}[ct][ct]{\matlabtextA $10$}%
\psfrag{005}[ct][ct]{\matlabtextA $11$}%
\psfrag{006}[ct][ct]{\matlabtextA $12$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextA $0$}%
\psfrag{008}[rc][rc]{\matlabtextA $10$}%
\psfrag{009}[rc][rc]{\matlabtextA $20$}%
\psfrag{010}[rc][rc]{\matlabtextA $30$}%
\psfrag{011}[rc][rc]{\matlabtextA $40$}%
\psfrag{012}[rc][rc]{\matlabtextA $50$}%
\psfrag{013}[rc][rc]{\matlabtextA $60$}%
\psfrag{014}[rc][rc]{\matlabtextA $70$}%
\psfrag{015}[rc][rc]{\matlabtextA $80$}%
%
%% </ytick>

==> d2.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{016}[cl][cl]{\matlabtextA $\tilde{S_{3}}$}%
\psfrag{017}[cl][cl]{\matlabtextA $\tilde{S_{2}}$}%
\psfrag{018}[cl][cl]{\matlabtextA $\tilde{S_{1}}$}%
\psfrag{019}[cl][cl]{\matlabtextA $\tilde{S_{0}}$}%
\psfrag{020}[cl][cl]{\matlabtextA Baseline scheme 2}%
\psfrag{021}[cl][cl]{\matlabtextA Proposed subopt. scheme}%
\psfrag{022}[cl][cl]{\matlabtextA Upper bound}%
\psfrag{023}[bc][bc]{\matlabtextA Average system sum throughput [bits/s/Hz]}%
\psfrag{024}[tc][tc]{\matlabtextA Delay $D$ (time slots)}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{025}[tl][tl]{\matlabtextB \begin{tabular}{@{}l@{}}Performance\\     gain\end{tabular}}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextB $1$}%
\psfrag{001}[ct][ct]{\matlabtextB $2$}%
\psfrag{002}[ct][ct]{\matlabtextB $3$}%
\psfrag{003}[ct][ct]{\matlabtextB $4$}%
\psfrag{004}[ct][ct]{\matlabtextB $5$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextB $0$}%
\psfrag{006}[rc][rc]{\matlabtextB $5$}%
\psfrag{007}[rc][rc]{\matlabtextB $10$}%
\psfrag{008}[rc][rc]{\matlabtextB $15$}%
\psfrag{009}[rc][rc]{\matlabtextB $20$}%
\psfrag{010}[rc][rc]{\matlabtextB $25$}%
\psfrag{011}[rc][rc]{\matlabtextB $30$}%
\psfrag{012}[rc][rc]{\matlabtextB $35$}%
\psfrag{013}[rc][rc]{\matlabtextB $40$}%
\psfrag{014}[rc][rc]{\matlabtextB $45$}%
\psfrag{015}[rc][rc]{\matlabtextB $50$}%
%
%% </ytick>

==> f1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{019}[cl][cl]{\matlabtextA Proposed subopt. scheme, $K=8$, $N_{T}=8$}%
\psfrag{020}[cl][cl]{\matlabtextA Proposed subopt. scheme, $K=6$, $N_{T}=6$}%
\psfrag{021}[cl][cl]{\matlabtextA Proposed subopt. scheme, $K=5$, $N_{T}=6$}%
\psfrag{022}[cl][cl]{\matlabtextA Proposed subopt. scheme, $K=4$, $N_{T}=6$}%
\psfrag{023}[bc][bc]{\matlabtextA System sum throughput [bits/s/Hz]}%
\psfrag{024}[tc][tc]{\matlabtextA Number of iterations}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $2$}%
\psfrag{001}[ct][ct]{\matlabtextA $4$}%
\psfrag{002}[ct][ct]{\matlabtextA $6$}%
\psfrag{003}[ct][ct]{\matlabtextA $8$}%
\psfrag{004}[ct][ct]{\matlabtextA $10$}%
\psfrag{005}[ct][ct]{\matlabtextA $12$}%
\psfrag{006}[ct][ct]{\matlabtextA $14$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextA $0$}%
\psfrag{008}[rc][rc]{\matlabtextA $5$}%
\psfrag{009}[rc][rc]{\matlabtextA $10$}%
\psfrag{010}[rc][rc]{\matlabtextA $15$}%
\psfrag{011}[rc][rc]{\matlabtextA $20$}%
\psfrag{012}[rc][rc]{\matlabtextA $25$}%
\psfrag{013}[rc][rc]{\matlabtextA $30$}%
\psfrag{014}[rc][rc]{\matlabtextA $35$}%
\psfrag{015}[rc][rc]{\matlabtextA $40$}%
\psfrag{016}[rc][rc]{\matlabtextA $45$}%
\psfrag{017}[rc][rc]{\matlabtextA $50$}%
\psfrag{018}[rc][rc]{\matlabtextA $55$}%
%
%% </ytick>

==> f1a.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{024}[cl][cl]{\matlabtextA Proposed subopt. scheme, $M=12$}%
\psfrag{025}[cl][cl]{\matlabtextA Proposed optimal scheme, $M=12$}%
\psfrag{026}[cl][cl]{\matlabtextA Proposed subopt. scheme, $M=16$}%
\psfrag{027}[cl][cl]{\matlabtextA Proposed optimal scheme, $M=16$}%
\psfrag{028}[bc][bc]{\matlabtextA System sum throughput [bits/s/Hz]}%
\psfrag{029}[tc][tc]{\matlabtextA Number of iterations}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $2$}%
\psfrag{001}[ct][ct]{\matlabtextB $4$}%
\psfrag{002}[ct][ct]{\matlabtextB $6$}%
\psfrag{003}[ct][ct]{\matlabtextB $8$}%
\psfrag{004}[ct][ct]{\matlabtextB $10$}%
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{009}[ct][ct]{\matlabtextC $500$}%
\psfrag{010}[ct][ct]{\matlabtextC $1000$}%
\psfrag{011}[ct][ct]{\matlabtextC $1500$}%
\psfrag{012}[ct][ct]{\matlabtextC $2000$}%
\psfrag{013}[ct][ct]{\matlabtextC $2500$}%
\psfrag{014}[ct][ct]{\matlabtextC $3000$}%
\psfrag{015}[ct][ct]{\matlabtextC $3500$}%
\psfrag{016}[ct][ct]{\matlabtextC $4000$}%
%
%% </xtick>
%
%% <ytick>
%
\providecommand\matlabtextD{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{005}[rc][rc]{\matlabtextD $10$}%
\psfrag{006}[rc][rc]{\matlabtextD $20$}%
\psfrag{007}[rc][rc]{\matlabtextD $30$}%
\psfrag{008}[rc][rc]{\matlabtextD $40$}%
%
\providecommand\matlabtextE{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{017}[rc][rc]{\matlabtextE $25$}%
\psfrag{018}[rc][rc]{\matlabtextE $30$}%
\psfrag{019}[rc][rc]{\matlabtextE $35$}%
\psfrag{020}[rc][rc]{\matlabtextE $40$}%
\psfrag{021}[rc][rc]{\matlabtextE $45$}%
\psfrag{022}[rc][rc]{\matlabtextE $50$}%
\psfrag{023}[rc][rc]{\matlabtextE $55$}%
%
%% </ytick>

==> f5.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{011}[cl][cl]{\matlabtextA Baseline 2}%
\psfrag{012}[cl][cl]{\matlabtextA Baseline 1}%
\psfrag{013}[cl][cl]{\matlabtextA Proposed subopt. scheme}%
\psfrag{014}[cl][cl]{\matlabtextA Proposed optimal scheme}%
\psfrag{015}[cl][cl]{\matlabtextA Upper bound}%
\psfrag{016}[bc][bc]{\matlabtextA Average system sum throughput [bits/s/Hz]}%
\psfrag{017}[tc][tc]{\matlabtextA Maximum transmit power of the BS [dBm]}%
\psfrag{019}[tl][tl]{\matlabtextA \begin{tabular}{@{}l@{}}Performance\\      gain\end{tabular}}%
\psfrag{020}[tl][tl]{\matlabtextA \begin{tabular}{@{}l@{}}Performance\\      gain\end{tabular}}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{11}{11}\selectfont\strut}%
\psfrag{018}[tl][tl]{\matlabtextB Performance gain}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $20$}%
\psfrag{001}[ct][ct]{\matlabtextC $25$}%
\psfrag{002}[ct][ct]{\matlabtextC $30$}%
\psfrag{003}[ct][ct]{\matlabtextC $35$}%
\psfrag{004}[ct][ct]{\matlabtextC $40$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $0$}%
\psfrag{006}[rc][rc]{\matlabtextC $5$}%
\psfrag{007}[rc][rc]{\matlabtextC $10$}%
\psfrag{008}[rc][rc]{\matlabtextC $15$}%
\psfrag{009}[rc][rc]{\matlabtextC $20$}%
\psfrag{010}[rc][rc]{\matlabtextC $25$}%
%
%% </ytick>

==> p1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{014}[cl][cl]{\matlabtextA $S_{1}, N_{T}=4$}%
\psfrag{015}[cl][cl]{\matlabtextA $S_{1}, N_{T}=8$}%
\psfrag{016}[cl][cl]{\matlabtextA $S_{0}, N_{T}=8$}%
\psfrag{017}[cl][cl]{\matlabtextA Baseline scheme 2}%
\psfrag{018}[cl][cl]{\matlabtextA Proposed subopt. scheme}%
\psfrag{019}[cl][cl]{\matlabtextA Upper bound}%
\psfrag{020}[bc][bc]{\matlabtextA Average system sum throughput [bits/s/Hz]}%
\psfrag{021}[tc][tc]{\matlabtextA Maximum transmit power of the BS [dBm]}%
\psfrag{022}[tl][tl]{\matlabtextA \begin{tabular}{@{}l@{}}Performance\\gain\\\end{tabular}}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $20$}%
\psfrag{001}[ct][ct]{\matlabtextA $25$}%
\psfrag{002}[ct][ct]{\matlabtextA $30$}%
\psfrag{003}[ct][ct]{\matlabtextA $35$}%
\psfrag{004}[ct][ct]{\matlabtextA $40$}%
\psfrag{005}[ct][ct]{\matlabtextA $45$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextA $0$}%
\psfrag{007}[rc][rc]{\matlabtextA $10$}%
\psfrag{008}[rc][rc]{\matlabtextA $20$}%
\psfrag{009}[rc][rc]{\matlabtextA $30$}%
\psfrag{010}[rc][rc]{\matlabtextA $40$}%
\psfrag{011}[rc][rc]{\matlabtextA $50$}%
\psfrag{012}[rc][rc]{\matlabtextA $60$}%
\psfrag{013}[rc][rc]{\matlabtextA $70$}%
%
%% </ytick>

==> u1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{016}[cl][cl]{\matlabtextA $S_{1}$}%
\psfrag{017}[cl][cl]{\matlabtextA $S_{0}$}%
\psfrag{018}[cl][cl]{\matlabtextA Baseline scheme 2}%
\psfrag{019}[cl][cl]{\matlabtextA Proposed subopt. scheme}%
\psfrag{020}[cl][cl]{\matlabtextA Upper bound}%
\psfrag{021}[bc][bc]{\matlabtextA Average system sum throughput [bits/s/Hz]}%
\psfrag{022}[tc][tc]{\matlabtextA Number of users}%
\psfrag{023}[tl][tl]{\matlabtextA \begin{tabular}{@{}l@{}}Performance\\      gain\end{tabular}}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $4$}%
\psfrag{001}[ct][ct]{\matlabtextA $5$}%
\psfrag{002}[ct][ct]{\matlabtextA $6$}%
\psfrag{003}[ct][ct]{\matlabtextA $7$}%
\psfrag{004}[ct][ct]{\matlabtextA $8$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextA $0$}%
\psfrag{006}[rc][rc]{\matlabtextA $10$}%
\psfrag{007}[rc][rc]{\matlabtextA $20$}%
\psfrag{008}[rc][rc]{\matlabtextA $30$}%
\psfrag{009}[rc][rc]{\matlabtextA $40$}%
\psfrag{010}[rc][rc]{\matlabtextA $50$}%
\psfrag{011}[rc][rc]{\matlabtextA $60$}%
\psfrag{012}[rc][rc]{\matlabtextA $70$}%
\psfrag{013}[rc][rc]{\matlabtextA $80$}%
\psfrag{014}[rc][rc]{\matlabtextA $90$}%
\psfrag{015}[rc][rc]{\matlabtextA $100$}%
%
%% </ytick>
